Evidence of a Past Merger of the Galactic Center Black Hole

The origin of supermassive black holes (SMBHs) residing in the centers of most galaxies remains a mystery. The Event Horizon Telescope (EHT) provided direct imaging of the SMBH Sgr A* at the Milky Way's center, indicating it likely spins rapidly with its spin axis significantly misaligned relative to the Galactic plane's angular momentum. Through investigating various SMBH growth models, here we show that the inferred spin properties of Sgr A* provide evidence of a past SMBH merger. Inspired by the merger between the Milky Way and Gaia-Enceladus, which has a 4:1 mass ratio as inferred from Gaia data, we have discovered that a 4:1 major merger of SMBH with a binary angular momentum inclination angle of 145-180 degrees with respect to the line of sight (LOS), can successfully replicate the measured spin properties of Sgr A*. This merger event in our galaxy provides potential observational support for the theory of hierarchical BH mergers in the formation and growth of SMBHs. The inferred merger rate, consistent with theoretical predictions, suggests a promising detection rate of SMBH mergers for space-borne gravitational wave detectors expected to operate in 2030s.

==> bib1.tex <==
\begin{thebibliography}{10}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}
\bibitem{Rechstone1998}
\bibinfo{author}{{Richstone}, D.} \emph{et~al.}
\newblock \bibinfo{title}{{Supermassive black holes and the evolution of galaxies.}}
\newblock \emph{\bibinfo{journal}{\nat}} \textbf{\bibinfo{volume}{385}}, \bibinfo{pages}{A14} (\bibinfo{year}{1998}).
\newblock \eprint{astro-ph/9810378}.

\bibitem{Fan2001}
\bibinfo{author}{{Fan}, X.} \emph{et~al.}
\newblock \bibinfo{title}{{A Survey of z$>$5.8 Quasars in the Sloan Digital Sky Survey. I. Discovery of Three New Quasars and the Spatial Density of Luminous Quasars at z\raisebox{-0.5ex}\textasciitilde6}}.
\newblock \emph{\bibinfo{journal}{\aj}} \textbf{\bibinfo{volume}{122}}, \bibinfo{pages}{2833--2849} (\bibinfo{year}{2001}).
\newblock \eprint{astro-ph/0108063}.

\bibitem{Lawrence2007}
\bibinfo{author}{{Lawrence}, A.} \emph{et~al.}
\newblock \bibinfo{title}{{The UKIRT Infrared Deep Sky Survey (UKIDSS)}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{379}}, \bibinfo{pages}{1599--1617} (\bibinfo{year}{2007}).
\newblock \eprint{astro-ph/0604426}.

\bibitem{Soltan1982}
\bibinfo{author}{{Soltan}, A.}
\newblock \bibinfo{title}{{Masses of quasars.}}
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{200}}, \bibinfo{pages}{115--122} (\bibinfo{year}{1982}).

\bibitem{Yu2002}
\bibinfo{author}{{Yu}, Q.} \& \bibinfo{author}{{Tremaine}, S.}
\newblock \bibinfo{title}{{Observational constraints on growth of massive black holes}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{335}}, \bibinfo{pages}{965--976} (\bibinfo{year}{2002}).
\newblock \eprint{astro-ph/0203082}.

\bibitem{Volonteri2003}
\bibinfo{author}{{Volonteri}, M.}, \bibinfo{author}{{Haardt}, F.} \& \bibinfo{author}{{Madau}, P.}
\newblock \bibinfo{title}{{The Assembly and Merging History of Supermassive Black Holes in Hierarchical Models of Galaxy Formation}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{582}}, \bibinfo{pages}{559--573} (\bibinfo{year}{2003}).
\newblock \eprint{astro-ph/0207276}.

\bibitem{Springel2005}
\bibinfo{author}{{Springel}, V.} \emph{et~al.}
\newblock \bibinfo{title}{{Simulations of the formation, evolution and clustering of galaxies and quasars}}.
\newblock \emph{\bibinfo{journal}{\nat}} \textbf{\bibinfo{volume}{435}}, \bibinfo{pages}{629--636} (\bibinfo{year}{2005}).
\newblock \eprint{astro-ph/0504097}.

\bibitem{EHTI2022}
\bibinfo{author}{{Event Horizon Telescope Collaboration}} \emph{et~al.}
\newblock \bibinfo{title}{{First Sagittarius A* Event Horizon Telescope Results. I. The Shadow of the Supermassive Black Hole in the Center of the Milky Way}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{930}}, \bibinfo{pages}{L12} (\bibinfo{year}{2022}).

\bibitem{Helmi2018}
\bibinfo{author}{{Helmi}, A.} \emph{et~al.}
\newblock \bibinfo{title}{{The merger that led to the formation of the Milky Way's inner stellar halo and thick disk}}.
\newblock \emph{\bibinfo{journal}{\nat}} \textbf{\bibinfo{volume}{563}}, \bibinfo{pages}{85--88} (\bibinfo{year}{2018}).
\newblock \eprint{1806.06038}.

\bibitem{LISA}
\bibinfo{author}{{Amaro-Seoane}, P.} \emph{et~al.}
\newblock \bibinfo{title}{{Laser Interferometer Space Antenna}}.
\newblock \emph{\bibinfo{journal}{arXiv e-prints}} \bibinfo{pages}{arXiv:1702.00786} (\bibinfo{year}{2017}).
\newblock \eprint{1702.00786}.

\bibitem{Taiji}
\bibinfo{author}{{Ruan}, W.-H.}, \bibinfo{author}{{Guo}, Z.-K.}, \bibinfo{author}{{Cai}, R.-G.} \& \bibinfo{author}{{Zhang}, Y.-Z.}
\newblock \bibinfo{title}{{Taiji Program: Gravitational-Wave Sources}}.
\newblock \emph{\bibinfo{journal}{arXiv e-prints}} \bibinfo{pages}{arXiv:1807.09495} (\bibinfo{year}{2018}).
\newblock \eprint{1807.09495}.

\bibitem{TianQin}
\bibinfo{author}{{Luo}, J.} \emph{et~al.}
\newblock \bibinfo{title}{{TianQin: a space-borne gravitational wave detector}}.
\newblock \emph{\bibinfo{journal}{Classical and Quantum Gravity}} \textbf{\bibinfo{volume}{33}}, \bibinfo{pages}{035010} (\bibinfo{year}{2016}).
\newblock \eprint{1512.02076}.

\bibitem{EHTV2022}
\bibinfo{author}{{Event Horizon Telescope Collaboration}} \emph{et~al.}
\newblock \bibinfo{title}{{First Sagittarius A* Event Horizon Telescope Results. V. Testing Astrophysical Models of the Galactic Center Black Hole}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{930}}, \bibinfo{pages}{L16} (\bibinfo{year}{2022}).

\bibitem{EHTVIII}
\bibinfo{author}{{Event Horizon Telescope Collaboration}} \emph{et~al.}
\newblock \bibinfo{title}{{First Sagittarius A* Event Horizon Telescope Results. VIII. Physical Interpretation of the Polarized Ring}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{964}}, \bibinfo{pages}{L26} (\bibinfo{year}{2024}).

\bibitem{Gravity2020b}
\bibinfo{author}{{GRAVITY Collaboration}} \emph{et~al.}
\newblock \bibinfo{title}{{Dynamically important magnetic fields near the event horizon of Sgr A*}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{643}}, \bibinfo{pages}{A56} (\bibinfo{year}{2020}).
\newblock \eprint{2009.01859}.

\bibitem{Fragione2020}
\bibinfo{author}{{Fragione}, G.} \& \bibinfo{author}{{Loeb}, A.}
\newblock \bibinfo{title}{{An Upper Limit on the Spin of SgrA* Based on Stellar Orbits in Its Vicinity}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{901}}, \bibinfo{pages}{L32} (\bibinfo{year}{2020}).
\newblock \eprint{2008.11734}.

\bibitem{Volonteri2007}
\bibinfo{author}{{Volonteri}, M.}, \bibinfo{author}{{Sikora}, M.} \& \bibinfo{author}{{Lasota}, J.-P.}
\newblock \bibinfo{title}{{Black Hole Spin and Galactic Morphology}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{667}}, \bibinfo{pages}{704--713} (\bibinfo{year}{2007}).
\newblock \eprint{0706.3900}.

\bibitem{King2006}
\bibinfo{author}{{King}, A.~R.} \& \bibinfo{author}{{Pringle}, J.~E.}
\newblock \bibinfo{title}{{Growing supermassive black holes by chaotic accretion}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{373}}, \bibinfo{pages}{L90--L92} (\bibinfo{year}{2006}).
\newblock \eprint{astro-ph/0609598}.

\bibitem{Dubois2014}
\bibinfo{author}{{Dubois}, Y.}, \bibinfo{author}{{Volonteri}, M.} \& \bibinfo{author}{{Silk}, J.}
\newblock \bibinfo{title}{{Black hole evolution - III. Statistical properties of mass growth and spin evolution using large-scale hydrodynamical cosmological simulations}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{440}}, \bibinfo{pages}{1590--1606} (\bibinfo{year}{2014}).
\newblock \eprint{1304.4583}.

\bibitem{Beckmann2022}
\bibinfo{author}{{Beckmann}, R.~S.} \emph{et~al.}
\newblock \bibinfo{title}{{Supermassive black holes in merger-free galaxies have higher spins which are preferentially aligned with their host galaxy}}.
\newblock \emph{\bibinfo{journal}{arXiv e-prints}} \bibinfo{pages}{arXiv:2211.13614} (\bibinfo{year}{2022}).
\newblock \eprint{2211.13614}.

\bibitem{Sala2023}
\bibinfo{author}{{Sala}, L.}, \bibinfo{author}{{Valentini}, M.}, \bibinfo{author}{{Biffi}, V.} \& \bibinfo{author}{{Dolag}, K.}
\newblock \bibinfo{title}{{Supermassive black hole spin evolution in cosmological simulations with OpenGadget3}}.
\newblock \emph{\bibinfo{journal}{arXiv e-prints}} \bibinfo{pages}{arXiv:2312.07657} (\bibinfo{year}{2023}).
\newblock \eprint{2312.07657}.

\bibitem{Peirani2024}
\bibinfo{author}{{Peirani}, S.} \emph{et~al.}
\newblock \bibinfo{title}{{Cosmic evolution of black hole-spin and galaxy orientations: clues from the NewHorizon and Galactica simulations}}.
\newblock \emph{\bibinfo{journal}{arXiv e-prints}} \bibinfo{pages}{arXiv:2401.03712} (\bibinfo{year}{2024}).
\newblock \eprint{2401.03712}.

\bibitem{Menou2001}
\bibinfo{author}{{Menou}, K.}, \bibinfo{author}{{Haiman}, Z.} \& \bibinfo{author}{{Narayanan}, V.~K.}
\newblock \bibinfo{title}{{The Merger History of Supermassive Black Holes in Galaxies}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{558}}, \bibinfo{pages}{535--542} (\bibinfo{year}{2001}).
\newblock \eprint{astro-ph/0101196}.

\bibitem{Tanaka2009}
\bibinfo{author}{{Tanaka}, T.} \& \bibinfo{author}{{Haiman}, Z.}
\newblock \bibinfo{title}{{The Assembly of Supermassive Black Holes at High Redshifts}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{696}}, \bibinfo{pages}{1798--1822} (\bibinfo{year}{2009}).
\newblock \eprint{0807.4702}.

\bibitem{Greene2020}
\bibinfo{author}{{Greene}, J.~E.}, \bibinfo{author}{{Strader}, J.} \& \bibinfo{author}{{Ho}, L.~C.}
\newblock \bibinfo{title}{{Intermediate-Mass Black Holes}}.
\newblock \emph{\bibinfo{journal}{\araa}} \textbf{\bibinfo{volume}{58}}, \bibinfo{pages}{257--312} (\bibinfo{year}{2020}).
\newblock \eprint{1911.09678}.

\bibitem{Blandford1977}
\bibinfo{author}{{Blandford}, R.~D.} \& \bibinfo{author}{{Znajek}, R.~L.}
\newblock \bibinfo{title}{{Electromagnetic extraction of energy from Kerr black holes.}}
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{179}}, \bibinfo{pages}{433--456} (\bibinfo{year}{1977}).

\bibitem{Lei2017}
\bibinfo{author}{{Lei}, W.-H.}, \bibinfo{author}{{Zhang}, B.}, \bibinfo{author}{{Wu}, X.-F.} \& \bibinfo{author}{{Liang}, E.-W.}
\newblock \bibinfo{title}{{Hyperaccreting Black Hole as Gamma-Ray Burst Central Engine. II. Temporal Evolution of the Central Engine Parameters during the Prompt and Afterglow Phases}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{849}}, \bibinfo{pages}{47} (\bibinfo{year}{2017}).
\newblock \eprint{1708.05043}.

\bibitem{Magorrian1998}
\bibinfo{author}{{Magorrian}, J.} \emph{et~al.}
\newblock \bibinfo{title}{{The Demography of Massive Dark Objects in Galaxy Centers}}.
\newblock \emph{\bibinfo{journal}{\aj}} \textbf{\bibinfo{volume}{115}}, \bibinfo{pages}{2285--2305} (\bibinfo{year}{1998}).
\newblock \eprint{astro-ph/9708072}.

\bibitem{Kormendy2013}
\bibinfo{author}{{Kormendy}, J.} \& \bibinfo{author}{{Ho}, L.~C.}
\newblock \bibinfo{title}{{Coevolution (Or Not) of Supermassive Black Holes and Host Galaxies}}.
\newblock \emph{\bibinfo{journal}{\araa}} \textbf{\bibinfo{volume}{51}}, \bibinfo{pages}{511--653} (\bibinfo{year}{2013}).
\newblock \eprint{1304.7762}.

\bibitem{Lang2013}
\bibinfo{author}{{Lang}, M.} \emph{et~al.}
\newblock \bibinfo{title}{{Can a satellite galaxy merger explain the active past of the Galactic Centre?}}
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{430}}, \bibinfo{pages}{2574--2584} (\bibinfo{year}{2013}).
\newblock \eprint{1107.2923}.

\bibitem{Schmitt2002}
\bibinfo{author}{{Schmitt}, H.~R.}, \bibinfo{author}{{Pringle}, J.~E.}, \bibinfo{author}{{Clarke}, C.~J.} \& \bibinfo{author}{{Kinney}, A.~L.}
\newblock \bibinfo{title}{{The Orientation of Jets Relative to Dust Disks in Radio Galaxies}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{575}}, \bibinfo{pages}{150--155} (\bibinfo{year}{2002}).
\newblock \eprint{astro-ph/0204247}.

\bibitem{Boylan2009}
\bibinfo{author}{{Boylan-Kolchin}, M.}, \bibinfo{author}{{Springel}, V.}, \bibinfo{author}{{White}, S. D.~M.}, \bibinfo{author}{{Jenkins}, A.} \& \bibinfo{author}{{Lemson}, G.}
\newblock \bibinfo{title}{{Resolving cosmic structure formation with the Millennium-II Simulation}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{398}}, \bibinfo{pages}{1150--1164} (\bibinfo{year}{2009}).
\newblock \eprint{0903.3041}.

\bibitem{Milosavljevic2001}
\bibinfo{author}{{Milosavljevi{\'c}}, M.} \& \bibinfo{author}{{Merritt}, D.}
\newblock \bibinfo{title}{{Formation of Galactic Nuclei}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{563}}, \bibinfo{pages}{34--62} (\bibinfo{year}{2001}).
\newblock \eprint{astro-ph/0103350}.

\bibitem{Sesana2015}
\bibinfo{author}{{Sesana}, A.} \& \bibinfo{author}{{Khan}, F.~M.}
\newblock \bibinfo{title}{{Scattering experiments meet N-body - I. A practical recipe for the evolution of massive black hole binaries in stellar environments}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{454}}, \bibinfo{pages}{L66--L70} (\bibinfo{year}{2015}).
\newblock \eprint{1505.02062}.

\bibitem{Ryu2018}
\bibinfo{author}{{Ryu}, T.}, \bibinfo{author}{{Perna}, R.}, \bibinfo{author}{{Haiman}, Z.}, \bibinfo{author}{{Ostriker}, J.~P.} \& \bibinfo{author}{{Stone}, N.~C.}
\newblock \bibinfo{title}{{Interactions between multiple supermassive black holes in galactic nuclei: a solution to the final parsec problem}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{473}}, \bibinfo{pages}{3410--3433} (\bibinfo{year}{2018}).
\newblock \eprint{1709.06501}.

\bibitem{Sesana2005}
\bibinfo{author}{{Sesana}, A.}, \bibinfo{author}{{Haardt}, F.}, \bibinfo{author}{{Madau}, P.} \& \bibinfo{author}{{Volonteri}, M.}
\newblock \bibinfo{title}{{The Gravitational Wave Signal from Massive Black Hole Binaries and Its Contribution to the LISA Data Stream}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{623}}, \bibinfo{pages}{23--30} (\bibinfo{year}{2005}).
\newblock \eprint{astro-ph/0409255}.

\bibitem{Volonteri2020}
\bibinfo{author}{{Volonteri}, M.} \emph{et~al.}
\newblock \bibinfo{title}{{Black hole mergers from dwarf to massive galaxies with the NewHorizon and Horizon-AGN simulations}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{498}}, \bibinfo{pages}{2219--2238} (\bibinfo{year}{2020}).
\newblock \eprint{2005.04902}.

\bibitem{Li2022}
\bibinfo{author}{{Li}, K.}, \bibinfo{author}{{Bogdanovi{\'c}}, T.}, \bibinfo{author}{{Ballantyne}, D.~R.} \& \bibinfo{author}{{Bonetti}, M.}
\newblock \bibinfo{title}{{Massive Black Hole Binaries from the TNG50-3 Simulation. I. Coalescence and LISA Detection Rates}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{933}}, \bibinfo{pages}{104} (\bibinfo{year}{2022}).
\newblock \eprint{2201.11088}.

\bibitem{Conselice2016}
\bibinfo{author}{{Conselice}, C.~J.}, \bibinfo{author}{{Wilkinson}, A.}, \bibinfo{author}{{Duncan}, K.} \& \bibinfo{author}{{Mortlock}, A.}
\newblock \bibinfo{title}{{The Evolution of Galaxy Number Density at z $<$ 8 and Its Implications}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{830}}, \bibinfo{pages}{83} (\bibinfo{year}{2016}).
\newblock \eprint{1607.03909}.

\bibitem{Reid2004}
\bibinfo{author}{{Reid}, M.~J.} \& \bibinfo{author}{{Brunthaler}, A.}
\newblock \bibinfo{title}{{The Proper Motion of Sagittarius A*. II. The Mass of Sagittarius A*}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{616}}, \bibinfo{pages}{872--884} (\bibinfo{year}{2004}).
\newblock \eprint{astro-ph/0408107}.

\bibitem{Ghez2008}
\bibinfo{author}{{Ghez}, A.~M.} \emph{et~al.}
\newblock \bibinfo{title}{{Measuring Distance and Properties of the Milky Way's Central Supermassive Black Hole with Stellar Orbits}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{689}}, \bibinfo{pages}{1044--1062} (\bibinfo{year}{2008}).
\newblock \eprint{0808.2870}.

\bibitem{Reid2020}
\bibinfo{author}{{Reid}, M.~J.} \& \bibinfo{author}{{Brunthaler}, A.}
\newblock \bibinfo{title}{{The Proper Motion of Sagittarius A*. III. The Case for a Supermassive Black Hole}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{892}}, \bibinfo{pages}{39} (\bibinfo{year}{2020}).
\newblock \eprint{2001.04386}.

\bibitem{Gualandris2008}
\bibinfo{author}{{Gualandris}, A.} \& \bibinfo{author}{{Merritt}, D.}
\newblock \bibinfo{title}{{Ejection of Supermassive Black Holes from Galaxy Cores}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{678}}, \bibinfo{pages}{780--797} (\bibinfo{year}{2008}).
\newblock \eprint{0708.0771}.

\end{thebibliography}


==> bib2.tex <==
\begin{thebibliography}{20}
		\setcounter{enumiv}{41}

\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}
\bibitem{Hirano2014}
\bibinfo{author}{{Hirano}, S.} \emph{et~al.}
\newblock \bibinfo{title}{{One Hundred First Stars: Protostellar Evolution and the Final Masses}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{781}}, \bibinfo{pages}{60} (\bibinfo{year}{2014}).
\newblock \eprint{1308.4456}.

\bibitem{Hirano2014}
\bibinfo{author}{{Hirano}, S.} \emph{et~al.}
\newblock \bibinfo{title}{{One Hundred First Stars: Protostellar Evolution and the Final Masses}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{781}}, \bibinfo{pages}{60} (\bibinfo{year}{2014}).
\newblock \eprint{1308.4456}.

\bibitem{Bond1984}
\bibinfo{author}{{Bond}, J.~R.}, \bibinfo{author}{{Arnett}, W.~D.} \& \bibinfo{author}{{Carr}, B.~J.}
\newblock \bibinfo{title}{{The evolution and fate of Very Massive Objects}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{280}}, \bibinfo{pages}{825--847} (\bibinfo{year}{1984}).

\bibitem{Madau2001}
\bibinfo{author}{{Madau}, P.} \& \bibinfo{author}{{Rees}, M.~J.}
\newblock \bibinfo{title}{{Massive Black Holes as Population III Remnants}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{551}}, \bibinfo{pages}{L27--L30} (\bibinfo{year}{2001}).
\newblock \eprint{astro-ph/0101223}.

\bibitem{Bahcall1975}
\bibinfo{author}{{Bahcall}, J.~N.} \& \bibinfo{author}{{Ostriker}, J.~P.}
\newblock \bibinfo{title}{{Massive black holes in globular clusters.}}
\newblock \emph{\bibinfo{journal}{\nat}} \textbf{\bibinfo{volume}{256}}, \bibinfo{pages}{23--24} (\bibinfo{year}{1975}).

\bibitem{Begelman1978}
\bibinfo{author}{{Begelman}, M.~C.} \& \bibinfo{author}{{Rees}, M.~J.}
\newblock \bibinfo{title}{{The fate of dense stellar systems}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{185}}, \bibinfo{pages}{847--860} (\bibinfo{year}{1978}).

\bibitem{Quinlan1990}
\bibinfo{author}{{Quinlan}, G.~D.} \& \bibinfo{author}{{Shapiro}, S.~L.}
\newblock \bibinfo{title}{{The Dynamical Evolution of Dense Star Clusters in Galactic Nuclei}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{356}}, \bibinfo{pages}{483} (\bibinfo{year}{1990}).

\bibitem{Lee1993}
\bibinfo{author}{{Lee}, M.~H.}
\newblock \bibinfo{title}{{N-Body Evolution of Dense Clusters of Compact Stars}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{418}}, \bibinfo{pages}{147} (\bibinfo{year}{1993}).

\bibitem{Ebisuzaki2001}
\bibinfo{author}{{Ebisuzaki}, T.} \emph{et~al.}
\newblock \bibinfo{title}{{Missing Link Found? The ``Runaway'' Path to Supermassive Black Holes}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{562}}, \bibinfo{pages}{L19--L22} (\bibinfo{year}{2001}).
\newblock \eprint{astro-ph/0106252}.

\bibitem{Miller2002}
\bibinfo{author}{{Miller}, M.~C.} \& \bibinfo{author}{{Hamilton}, D.~P.}
\newblock \bibinfo{title}{{Production of intermediate-mass black holes in globular clusters}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{330}}, \bibinfo{pages}{232--240} (\bibinfo{year}{2002}).
\newblock \eprint{astro-ph/0106188}.

\bibitem{Portegies2002}
\bibinfo{author}{{Portegies Zwart}, S.~F.} \& \bibinfo{author}{{McMillan}, S. L.~W.}
\newblock \bibinfo{title}{{The Runaway Growth of Intermediate-Mass Black Holes in Dense Star Clusters}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{576}}, \bibinfo{pages}{899--907} (\bibinfo{year}{2002}).
\newblock \eprint{astro-ph/0201055}.

\bibitem{Rose2022}
\bibinfo{author}{{Rose}, S.~C.}, \bibinfo{author}{{Naoz}, S.}, \bibinfo{author}{{Sari}, R.} \& \bibinfo{author}{{Linial}, I.}
\newblock \bibinfo{title}{{The Formation of Intermediate-mass Black Holes in Galactic Nuclei}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{929}}, \bibinfo{pages}{L22} (\bibinfo{year}{2022}).
\newblock \eprint{2201.00022}.

\bibitem{Atallah2023}
\bibinfo{author}{{Atallah}, D.} \emph{et~al.}
\newblock \bibinfo{title}{{Growing black holes through successive mergers in galactic nuclei - I. Methods and first results}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{523}}, \bibinfo{pages}{4227--4250} (\bibinfo{year}{2023}).
\newblock \eprint{2211.09670}.

\bibitem{Omukai2008}
\bibinfo{author}{{Omukai}, K.}, \bibinfo{author}{{Schneider}, R.} \& \bibinfo{author}{{Haiman}, Z.}
\newblock \bibinfo{title}{{Can Supermassive Black Holes Form in Metal-enriched High-Redshift Protogalaxies?}}
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{686}}, \bibinfo{pages}{801--814} (\bibinfo{year}{2008}).
\newblock \eprint{0804.3141}.

\bibitem{Devecchi2009}
\bibinfo{author}{{Devecchi}, B.} \& \bibinfo{author}{{Volonteri}, M.}
\newblock \bibinfo{title}{{Formation of the First Nuclear Clusters and Massive Black Holes at High Redshift}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{694}}, \bibinfo{pages}{302--313} (\bibinfo{year}{2009}).
\newblock \eprint{0810.1057}.

\bibitem{Loeb1994}
\bibinfo{author}{{Loeb}, A.} \& \bibinfo{author}{{Rasio}, F.~A.}
\newblock \bibinfo{title}{{Collapse of Primordial Gas Clouds and the Formation of Quasar Black Holes}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{432}}, \bibinfo{pages}{52} (\bibinfo{year}{1994}).
\newblock \eprint{astro-ph/9401026}.

\bibitem{Begelman2006}
\bibinfo{author}{{Begelman}, M.~C.}, \bibinfo{author}{{Volonteri}, M.} \& \bibinfo{author}{{Rees}, M.~J.}
\newblock \bibinfo{title}{{Formation of supermassive black holes by direct collapse in pre-galactic haloes}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{370}}, \bibinfo{pages}{289--298} (\bibinfo{year}{2006}).
\newblock \eprint{astro-ph/0602363}.

\bibitem{Lodato2006}
\bibinfo{author}{{Lodato}, G.} \& \bibinfo{author}{{Natarajan}, P.}
\newblock \bibinfo{title}{{Supermassive black hole formation during the assembly of pre-galactic discs}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{371}}, \bibinfo{pages}{1813--1823} (\bibinfo{year}{2006}).
\newblock \eprint{astro-ph/0606159}.

\bibitem{Shakura1973}
\bibinfo{author}{{Shakura}, N.~I.} \& \bibinfo{author}{{Sunyaev}, R.~A.}
\newblock \bibinfo{title}{{Black holes in binary systems. Observational appearance.}}
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{24}}, \bibinfo{pages}{337--355} (\bibinfo{year}{1973}).

\bibitem{Lynden1974}
\bibinfo{author}{{Lynden-Bell}, D.} \& \bibinfo{author}{{Pringle}, J.~E.}
\newblock \bibinfo{title}{{The evolution of viscous discs and the origin of the nebular variables.}}
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{168}}, \bibinfo{pages}{603--637} (\bibinfo{year}{1974}).

\bibitem{Shapiro1976}
\bibinfo{author}{{Shapiro}, S.~L.}, \bibinfo{author}{{Lightman}, A.~P.} \& \bibinfo{author}{{Eardley}, D.~M.}
\newblock \bibinfo{title}{{A two-temperature accretion disk model for Cygnus X-1: structure and spectrum.}}
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{204}}, \bibinfo{pages}{187--199} (\bibinfo{year}{1976}).

\bibitem{Ichimaru1977}
\bibinfo{author}{{Ichimaru}, S.}
\newblock \bibinfo{title}{{Bimodal behavior of accretion disks: theory and application to Cygnus X-1 transitions.}}
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{214}}, \bibinfo{pages}{840--855} (\bibinfo{year}{1977}).

\bibitem{Narayan1994}
\bibinfo{author}{{Narayan}, R.} \& \bibinfo{author}{{Yi}, I.}
\newblock \bibinfo{title}{{Advection-dominated Accretion: A Self-similar Solution}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{428}}, \bibinfo{pages}{L13} (\bibinfo{year}{1994}).
\newblock \eprint{astro-ph/9403052}.

\bibitem{Narayan1995}
\bibinfo{author}{{Narayan}, R.} \& \bibinfo{author}{{Yi}, I.}
\newblock \bibinfo{title}{{Advection-dominated Accretion: Self-Similarity and Bipolar Outflows}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{444}}, \bibinfo{pages}{231} (\bibinfo{year}{1995}).
\newblock \eprint{astro-ph/9411058}.

\bibitem{Blandford1999}
\bibinfo{author}{{Blandford}, R.~D.} \& \bibinfo{author}{{Begelman}, M.~C.}
\newblock \bibinfo{title}{{On the fate of gas accreting at a low rate on to a black hole}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{303}}, \bibinfo{pages}{L1--L5} (\bibinfo{year}{1999}).
\newblock \eprint{astro-ph/9809083}.

\bibitem{McKinney}
\bibinfo{author}{{McKinney}, J.~C.}
\newblock \bibinfo{title}{{Total and Jet Blandford-Znajek Power in the Presence of an Accretion Disk}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{630}}, \bibinfo{pages}{L5--L8} (\bibinfo{year}{2005}).
\newblock \eprint{astro-ph/0506367}.

\bibitem{Ghisellini2014}
\bibinfo{author}{{Ghisellini}, G.}, \bibinfo{author}{{Tavecchio}, F.}, \bibinfo{author}{{Maraschi}, L.}, \bibinfo{author}{{Celotti}, A.} \& \bibinfo{author}{{Sbarrato}, T.}
\newblock \bibinfo{title}{{The power of relativistic jets is larger than the luminosity of their accretion disks}}.
\newblock \emph{\bibinfo{journal}{\nat}} \textbf{\bibinfo{volume}{515}}, \bibinfo{pages}{376--378} (\bibinfo{year}{2014}).
\newblock \eprint{1411.5368}.

\bibitem{Narayan2022}
\bibinfo{author}{{Narayan}, R.}, \bibinfo{author}{{Chael}, A.}, \bibinfo{author}{{Chatterjee}, K.}, \bibinfo{author}{{Ricarte}, A.} \& \bibinfo{author}{{Curd}, B.}
\newblock \bibinfo{title}{{Jets in magnetically arrested hot accretion flows: geometry, power, and black hole spin-down}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{511}}, \bibinfo{pages}{3795--3813} (\bibinfo{year}{2022}).
\newblock \eprint{2108.12380}.

\bibitem{Igumenshchev2003}
\bibinfo{author}{{Igumenshchev}, I.~V.}, \bibinfo{author}{{Narayan}, R.} \& \bibinfo{author}{{Abramowicz}, M.~A.}
\newblock \bibinfo{title}{{Three-dimensional Magnetohydrodynamic Simulations of Radiatively Inefficient Accretion Flows}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{592}}, \bibinfo{pages}{1042--1059} (\bibinfo{year}{2003}).
\newblock \eprint{astro-ph/0301402}.

\bibitem{Narayan2003}
\bibinfo{author}{{Narayan}, R.}, \bibinfo{author}{{Igumenshchev}, I.~V.} \& \bibinfo{author}{{Abramowicz}, M.~A.}
\newblock \bibinfo{title}{{Magnetically Arrested Disk: an Energetically Efficient Accretion Flow}}.
\newblock \emph{\bibinfo{journal}{\pasj}} \textbf{\bibinfo{volume}{55}}, \bibinfo{pages}{L69--L72} (\bibinfo{year}{2003}).
\newblock \eprint{astro-ph/0305029}.

\bibitem{Narayan2012b}
\bibinfo{author}{{Narayan}, R.}, \bibinfo{author}{{S{\"A} dowski}, A.}, \bibinfo{author}{{Penna}, R.~F.} \& \bibinfo{author}{{Kulkarni}, A.~K.}
\newblock \bibinfo{title}{{GRMHD simulations of magnetized advection-dominated accretion on a non-spinning black hole: role of outflows}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{426}}, \bibinfo{pages}{3241--3259} (\bibinfo{year}{2012}).
\newblock \eprint{1206.1213}.

\bibitem{Page1974}
\bibinfo{author}{{Page}, D.~N.} \& \bibinfo{author}{{Thorne}, K.~S.}
\newblock \bibinfo{title}{{Disk-Accretion onto a Black Hole. Time-Averaged Structure of Accretion Disk}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{191}}, \bibinfo{pages}{499--506} (\bibinfo{year}{1974}).

\bibitem{King2008}
\bibinfo{author}{{King}, A.~R.}, \bibinfo{author}{{Pringle}, J.~E.} \& \bibinfo{author}{{Hofmann}, J.~A.}
\newblock \bibinfo{title}{{The evolution of black hole mass and spin in active galactic nuclei}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{385}}, \bibinfo{pages}{1621--1627} (\bibinfo{year}{2008}).
\newblock \eprint{0801.1564}.

\bibitem{Chen2023}
\bibinfo{author}{{Chen}, Y.-X.} \& \bibinfo{author}{{Lin}, D. N.~C.}
\newblock \bibinfo{title}{{Chaotic gas accretion by black holes embedded in AGN discs as cause of low-spin signatures in gravitational wave events}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{522}}, \bibinfo{pages}{319--329} (\bibinfo{year}{2023}).
\newblock \eprint{2303.17097}.

\bibitem{Bustamante2019}
\bibinfo{author}{{Bustamante}, S.} \& \bibinfo{author}{{Springel}, V.}
\newblock \bibinfo{title}{{Spin evolution and feedback of supermassive black holes in cosmological simulations}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{490}}, \bibinfo{pages}{4133--4153} (\bibinfo{year}{2019}).
\newblock \eprint{1902.04651}.

\bibitem{Varma2019b}
\bibinfo{author}{{Varma}, V.} \emph{et~al.}
\newblock \bibinfo{title}{{Surrogate models for precessing binary black hole simulations with unequal masses}}.
\newblock \emph{\bibinfo{journal}{Physical Review Research}} \textbf{\bibinfo{volume}{1}}, \bibinfo{pages}{033015} (\bibinfo{year}{2019}).
\newblock \eprint{1905.09300}.

\bibitem{Boschini2023}
\bibinfo{author}{{Boschini}, M.} \emph{et~al.}
\newblock \bibinfo{title}{{Extending black-hole remnant surrogate models to extreme mass ratios}}.
\newblock \emph{\bibinfo{journal}{\prd}} \textbf{\bibinfo{volume}{108}}, \bibinfo{pages}{084015} (\bibinfo{year}{2023}).
\newblock \eprint{2307.03435}.

\bibitem{Blackman2017}
\bibinfo{author}{{Blackman}, J.} \emph{et~al.}
\newblock \bibinfo{title}{{Numerical relativity waveform surrogate model for generically precessing binary black hole mergers}}.
\newblock \emph{\bibinfo{journal}{\prd}} \textbf{\bibinfo{volume}{96}}, \bibinfo{pages}{024058} (\bibinfo{year}{2017}).
\newblock \eprint{1705.07089}.

\bibitem{Varma2019}
\bibinfo{author}{{Varma}, V.}, \bibinfo{author}{{Gerosa}, D.}, \bibinfo{author}{{Stein}, L.~C.}, \bibinfo{author}{{H{\'e}bert}, F.} \& \bibinfo{author}{{Zhang}, H.}
\newblock \bibinfo{title}{{High-Accuracy Mass, Spin, and Recoil Predictions of Generic Black-Hole Merger Remnants}}.
\newblock \emph{\bibinfo{journal}{\prl}} \textbf{\bibinfo{volume}{122}}, \bibinfo{pages}{011101} (\bibinfo{year}{2019}).
\newblock \eprint{1809.09125}.

\bibitem{Guo2011}
\bibinfo{author}{{Guo}, Q.} \emph{et~al.}
\newblock \bibinfo{title}{{From dwarf spheroidals to cD galaxies: simulating the galaxy population in a {\ensuremath{\Lambda}}CDM cosmology}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{413}}, \bibinfo{pages}{101--131} (\bibinfo{year}{2011}).
\newblock \eprint{1006.0106}.

\bibitem{Thorp2018}
\bibinfo{author}{{Thorp}, S.}, \bibinfo{author}{{Chadwick}, E.} \& \bibinfo{author}{{Sesana}, A.}
\newblock \bibinfo{title}{{Tidal disruption events from massive black hole binaries: predictions for ongoing and future surveys}}.
\newblock \emph{\bibinfo{journal}{arXiv e-prints}} \bibinfo{pages}{arXiv:1811.01960} (\bibinfo{year}{2018}).
\newblock \eprint{1811.01960}.

\bibitem{Begelman1980}
\bibinfo{author}{{Begelman}, M.~C.}, \bibinfo{author}{{Blandford}, R.~D.} \& \bibinfo{author}{{Rees}, M.~J.}
\newblock \bibinfo{title}{{Massive black hole binaries in active galactic nuclei}}.
\newblock \emph{\bibinfo{journal}{\nat}} \textbf{\bibinfo{volume}{287}}, \bibinfo{pages}{307--309} (\bibinfo{year}{1980}).

\bibitem{Goldreich1980}
\bibinfo{author}{{Goldreich}, P.} \& \bibinfo{author}{{Tremaine}, S.}
\newblock \bibinfo{title}{{Disk-satellite interactions.}}
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{241}}, \bibinfo{pages}{425--441} (\bibinfo{year}{1980}).

\bibitem{Berczik2006}
\bibinfo{author}{{Berczik}, P.}, \bibinfo{author}{{Merritt}, D.}, \bibinfo{author}{{Spurzem}, R.} \& \bibinfo{author}{{Bischof}, H.-P.}
\newblock \bibinfo{title}{{Efficient Merger of Binary Supermassive Black Holes in Nonaxisymmetric Galaxies}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{642}}, \bibinfo{pages}{L21--L24} (\bibinfo{year}{2006}).
\newblock \eprint{astro-ph/0601698}.

\bibitem{Vasiliev2015}
\bibinfo{author}{{Vasiliev}, E.}, \bibinfo{author}{{Antonini}, F.} \& \bibinfo{author}{{Merritt}, D.}
\newblock \bibinfo{title}{{The Final-parsec Problem in the Collisionless Limit}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{810}}, \bibinfo{pages}{49} (\bibinfo{year}{2015}).
\newblock \eprint{1505.05480}.

\bibitem{Quinlan1996}
\bibinfo{author}{{Quinlan}, G.~D.}
\newblock \bibinfo{title}{{The dynamical evolution of massive black hole binaries I. Hardening in a fixed stellar background}}.
\newblock \emph{\bibinfo{journal}{\na}} \textbf{\bibinfo{volume}{1}}, \bibinfo{pages}{35--56} (\bibinfo{year}{1996}).
\newblock \eprint{astro-ph/9601092}.

\bibitem{Sesana2006}
\bibinfo{author}{{Sesana}, A.}, \bibinfo{author}{{Haardt}, F.} \& \bibinfo{author}{{Madau}, P.}
\newblock \bibinfo{title}{{Interaction of Massive Black Hole Binaries with Their Stellar Environment. I. Ejection of Hypervelocity Stars}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{651}}, \bibinfo{pages}{392--400} (\bibinfo{year}{2006}).
\newblock \eprint{astro-ph/0604299}.

\bibitem{Peters1963}
\bibinfo{author}{{Peters}, P.~C.} \& \bibinfo{author}{{Mathews}, J.}
\newblock \bibinfo{title}{{Gravitational Radiation from Point Masses in a Keplerian Orbit}}.
\newblock \emph{\bibinfo{journal}{Physical Review}} \textbf{\bibinfo{volume}{131}}, \bibinfo{pages}{435--440} (\bibinfo{year}{1963}).

\bibitem{Peters1964}
\bibinfo{author}{{Peters}, P.~C.}
\newblock \bibinfo{title}{{Gravitational Radiation and the Motion of Two Point Masses}}.
\newblock \emph{\bibinfo{journal}{Physical Review}} \textbf{\bibinfo{volume}{136}}, \bibinfo{pages}{1224--1232} (\bibinfo{year}{1964}).

\bibitem{Dehnen1993}
\bibinfo{author}{{Dehnen}, W.}
\newblock \bibinfo{title}{{A Family of Potential-Density Pairs for Spherical Galaxies and Bulges}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{265}}, \bibinfo{pages}{250} (\bibinfo{year}{1993}).

\bibitem{Dabringhausen2008}
\bibinfo{author}{{Dabringhausen}, J.}, \bibinfo{author}{{Hilker}, M.} \& \bibinfo{author}{{Kroupa}, P.}
\newblock \bibinfo{title}{{From star clusters to dwarf galaxies: the properties of dynamically hot stellar systems}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{386}}, \bibinfo{pages}{864--886} (\bibinfo{year}{2008}).
\newblock \eprint{0802.0703}.

\bibitem{Bekenstein1973}
\bibinfo{author}{{Bekenstein}, J.~D.}
\newblock \bibinfo{title}{{Gravitational-Radiation Recoil and Runaway Black Holes}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{183}}, \bibinfo{pages}{657--664} (\bibinfo{year}{1973}).

\bibitem{Blecha2008}
\bibinfo{author}{{Blecha}, L.} \& \bibinfo{author}{{Loeb}, A.}
\newblock \bibinfo{title}{{Effects of gravitational-wave recoil on the dynamics and growth of supermassive black holes}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{390}}, \bibinfo{pages}{1311--1325} (\bibinfo{year}{2008}).
\newblock \eprint{0805.1420}.

\bibitem{Merritt2007}
\bibinfo{author}{{Merritt}, D.}, \bibinfo{author}{{Berczik}, P.} \& \bibinfo{author}{{Laun}, F.}
\newblock \bibinfo{title}{{Brownian Motion of Black Holes in Dense Nuclei}}.
\newblock \emph{\bibinfo{journal}{\aj}} \textbf{\bibinfo{volume}{133}}, \bibinfo{pages}{553--563} (\bibinfo{year}{2007}).
\newblock \eprint{astro-ph/0408029}.

\bibitem{Hansen2003}
\bibinfo{author}{{Hansen}, B. M.~S.} \& \bibinfo{author}{{Milosavljevi{\'c}}, M.}
\newblock \bibinfo{title}{{The Need for a Second Black Hole at the Galactic Center}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{593}}, \bibinfo{pages}{L77--L80} (\bibinfo{year}{2003}).
\newblock \eprint{astro-ph/0306074}.

\bibitem{Maillard2004}
\bibinfo{author}{{Maillard}, J.~P.}, \bibinfo{author}{{Paumard}, T.}, \bibinfo{author}{{Stolovy}, S.~R.} \& \bibinfo{author}{{Rigaut}, F.}
\newblock \bibinfo{title}{{The nature of the Galactic Center source IRS 13 revealed by high spatial resolution in the infrared}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{423}}, \bibinfo{pages}{155--167} (\bibinfo{year}{2004}).
\newblock \eprint{astro-ph/0404450}.

\bibitem{Gurkan2005}
\bibinfo{author}{{G{\"u}rkan}, M.~A.} \& \bibinfo{author}{{Rasio}, F.~A.}
\newblock \bibinfo{title}{{The Disruption of Stellar Clusters Containing Massive Black Holes near the Galactic Center}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{628}}, \bibinfo{pages}{236--245} (\bibinfo{year}{2005}).
\newblock \eprint{astro-ph/0412452}.

\bibitem{Gualandris2009}
\bibinfo{author}{{Gualandris}, A.} \& \bibinfo{author}{{Merritt}, D.}
\newblock \bibinfo{title}{{Perturbations of Intermediate-mass Black Holes on Stellar Orbits in the Galactic Center}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{705}}, \bibinfo{pages}{361--371} (\bibinfo{year}{2009}).
\newblock \eprint{0905.4514}.

\bibitem{Chen2013}
\bibinfo{author}{{Chen}, X.} \& \bibinfo{author}{{Liu}, F.~K.}
\newblock \bibinfo{title}{{Is There an Intermediate Massive Black Hole in the Galactic Center: Imprints on the Stellar Tidal-disruption Rate}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{762}}, \bibinfo{pages}{95} (\bibinfo{year}{2013}).
\newblock \eprint{1211.4609}.

\bibitem{Generozov2020}
\bibinfo{author}{{Generozov}, A.} \& \bibinfo{author}{{Madigan}, A.-M.}
\newblock \bibinfo{title}{{The Hills Mechanism and the Galactic Center S-stars}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{896}}, \bibinfo{pages}{137} (\bibinfo{year}{2020}).
\newblock \eprint{2002.10547}.

\bibitem{Naoz2020}
\bibinfo{author}{{Naoz}, S.} \emph{et~al.}
\newblock \bibinfo{title}{{A Hidden Friend for the Galactic Center Black Hole, Sgr A*}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{888}}, \bibinfo{pages}{L8} (\bibinfo{year}{2020}).
\newblock \eprint{1912.04910}.

\bibitem{Zheng2020}
\bibinfo{author}{{Zheng}, X.}, \bibinfo{author}{{Lin}, D. N.~C.} \& \bibinfo{author}{{Mao}, S.}
\newblock \bibinfo{title}{{The Influence of the Secular Perturbation of an Intermediate-mass Companion. I. Eccentricity Excitation of Disk Stars at the Galactic Center}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{905}}, \bibinfo{pages}{169} (\bibinfo{year}{2020}).
\newblock \eprint{2011.04653}.

\bibitem{RoseNaoz2022}
\bibinfo{author}{{Rose}, S.~C.}, \bibinfo{author}{{Naoz}, S.}, \bibinfo{author}{{Sari}, R.} \& \bibinfo{author}{{Linial}, I.}
\newblock \bibinfo{title}{{The Formation of Intermediate-mass Black Holes in Galactic Nuclei}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{929}}, \bibinfo{pages}{L22} (\bibinfo{year}{2022}).
\newblock \eprint{2201.00022}.

\bibitem{Will2023}
\bibinfo{author}{{Will}, C.~M.} \emph{et~al.}
\newblock \bibinfo{title}{{Constraining a Companion of the Galactic Center Black Hole Sgr A*}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{959}}, \bibinfo{pages}{58} (\bibinfo{year}{2023}).
\newblock \eprint{2307.16646}.

\bibitem{Gravity2023}
\bibinfo{author}{{Gravity Collaboration}} \emph{et~al.}
\newblock \bibinfo{title}{{Where intermediate-mass black holes could hide in the Galactic Centre. A full parameter study with the S2 orbit}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{672}}, \bibinfo{pages}{A63} (\bibinfo{year}{2023}).
\newblock \eprint{2303.04067}.

\end{thebibliography}

